Power-based Safety Layer for Aerial Vehicles in Physical Interaction using Lyapunov Exponents

As the performance of autonomous systems increases, safety concerns arise, especially when operating in non-structured environments. To deal with these concerns, this work presents a safety layer for mechanical systems that detects and responds to unstable dynamics caused by external disturbances. The safety layer is implemented independently and on top of already present nominal controllers, like pose or wrench tracking, and limits power flow when the system's response would lead to instability. This approach is based on the computation of the Largest Lyapunov Exponent (LLE) of the system's error dynamics, which represent a measure of the dynamics' divergence or convergence rate. By actively computing this metric, divergent and possibly dangerous system behaviors can be promptly detected. The LLE is then used in combination with Control Barrier Functions (CBFs) to impose power limit constraints on a jerk controlled system. The proposed architecture is experimentally validated on an Omnidirectional Micro Aerial Vehicle (OMAV) both in free flight and interaction tasks.

==> mathsym.tex <==
%%%%%%% PACKAGES
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

%%%%%%% Mathematical Symbols ==>>
\def\tr{^{\rm T}}
\def\trd{{}^{\rm T}}
\def\minustr{{}^{-\rm T}}
\def\Atan{\mathrm{Atan2}}
\def\Acos{\mathrm{Acos}}
\def\sgn{\mathrm{sgn}}
\def\de{\mathrm{d}}
\def\pde{\partial}
\def\diag{\mathrm{diag}}
\newcommand{\inv}{^{-1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\skewMat}[1]{\left[#1\right]_{\times}}
\newcommand{\SE}{\textnormal{SE}}

\def\zero{\hbox{\bf 0}}
\def\Zero{{\mbox{\boldmath $O$}}}

\def\bfa{{\mbox{\boldmath $a$}}}
\def\bfb{{\mbox{\boldmath $b$}}}
\def\bfc{{\mbox{\boldmath $c$}}}
\def\bfd{{\mbox{\boldmath $d$}}}
\def\bfe{{\mbox{\boldmath $e$}}}
\def\bff{{\mbox{\boldmath $f$}}}
\def\bfg{{\mbox{\boldmath $g$}}}
\def\bfh{{\mbox{\boldmath $h$}}}
\def\bfi{{\mbox{\boldmath $i$}}}
\def\bfj{{\mbox{\boldmath $j$}}}
\def\bfk{{\mbox{\boldmath $k$}}}
\def\bfl{{\mbox{\boldmath $l$}}}
\def\bfm{{\mbox{\boldmath $m$}}}
\def\bfn{{\mbox{\boldmath $n$}}}
\def\bfo{{\mbox{\boldmath $o$}}}
\def\bfp{{\mbox{\boldmath $p$}}}
\def\bfq{{\mbox{\boldmath $q$}}}
\def\bfr{{\mbox{\boldmath $r$}}}
\def\bfs{{\mbox{\boldmath $s$}}}
\def\bft{{\mbox{\boldmath $t$}}}
\def\bfu{{\mbox{\boldmath $u$}}}
\def\bfv{{\mbox{\boldmath $v$}}}
\def\bfw{{\mbox{\boldmath $w$}}}
\def\bfx{{\mbox{\boldmath $x$}}}
\def\bfy{{\mbox{\boldmath $y$}}}
\def\bfz{{\mbox{\boldmath $z$}}}

\def\bfA{{\mbox{\boldmath $A$}}}
\def\bfB{{\mbox{\boldmath $B$}}}
\def\bfC{{\mbox{\boldmath $C$}}}
\def\bfD{{\mbox{\boldmath $D$}}}
\def\bfE{{\mbox{\boldmath $E$}}}
\def\bfF{{\mbox{\boldmath $F$}}}
\def\bfG{{\mbox{\boldmath $G$}}}
\def\bfH{{\mbox{\boldmath $H$}}}
\def\bfI{{\mbox{\boldmath $I$}}}
\def\bfJ{{\mbox{\boldmath $J$}}}
\def\bfK{{\mbox{\boldmath $K$}}}
\def\bfL{{\mbox{\boldmath $L$}}}
\def\bfM{{\mbox{\boldmath $M$}}}
\def\bfN{{\mbox{\boldmath $N$}}}
\def\bfO{{\mbox{\boldmath $O$}}}
\def\bfP{{\mbox{\boldmath $P$}}}
\def\bfQ{{\mbox{\boldmath $Q$}}}
\def\bfR{{\mbox{\boldmath $R$}}}
\def\bfS{{\mbox{\boldmath $S$}}}
\def\bfT{{\mbox{\boldmath $T$}}}
\def\bfU{{\mbox{\boldmath $U$}}}
\def\bfV{{\mbox{\boldmath $V$}}}
\def\bfW{{\mbox{\boldmath $W$}}}
\def\bfX{{\mbox{\boldmath $X$}}}
\def\bfY{{\mbox{\boldmath $Y$}}}
\def\bfZ{{\mbox{\boldmath $Z$}}}

\def\bfGamma{{\mbox{\boldmath $\Gamma$}}}
\def\bfDelta{{\mbox{\boldmath $\Delta$}}}
\def\bfTheta{{\mbox{\boldmath $\Theta$}}}
\def\bfLambda{{\mbox{\boldmath $\Lambda$}}}
\def\bfXi{{\mbox{\boldmath $\Xi$}}}
\def\bfPi{{\mbox{\boldmath $\Pi$}}}
\def\bfSigma{{\mbox{\boldmath $\Sigma$}}}
\def\bfUpsilon{{\mbox{\boldmath $\Upsilon$}}}
\def\bfPhi{{\mbox{\boldmath $\Phi$}}}
\def\bfPsi{{\mbox{\boldmath $\Psi$}}}
\def\bfOmega{{\mbox{\boldmath $\Omega$}}}
\def\bfalpha{{\mbox{\boldmath $\alpha$}}}
\def\bfbeta{{\mbox{\boldmath $\beta$}}}
\def\bfgamma{{\mbox{\boldmath $\gamma$}}}
\def\bfdelta{{\mbox{\boldmath $\delta$}}}
\def\bfepsilon{{\mbox{\boldmath $\epsilon$}}}
\def\bfzeta{{\mbox{\boldmath $\zeta$}}}
\def\bfeta{{\mbox{\boldmath $\eta$}}}
\def\bftheta{{\mbox{\boldmath $\theta$}}}
\def\bfiota{{\mbox{\boldmath $\iota$}}}
\def\bfkappa{{\mbox{\boldmath $\kappa$}}}
\def\bflambda{{\mbox{\boldmath $\lambda$}}}
\def\bfmu{{\mbox{\boldmath $\mu$}}}
\def\bfnu{{\mbox{\boldmath $\nu$}}}
\def\bfxi{{\mbox{\boldmath $\xi$}}}
\def\bfpi{{\mbox{\boldmath $\pi$}}}
\def\bfrho{{\mbox{\boldmath $\rho$}}}
\def\bfsigma{{\mbox{\boldmath $\sigma$}}}
\def\bftau{{\mbox{\boldmath $\tau$}}}
\def\bfupsilon{{\mbox{\boldmath $\upsilon$}}}
\def\bfphi{{\mbox{\boldmath $\phi$}}}
\def\bfchi{{\mbox{\boldmath $\chi$}}}
\def\bfpsi{{\mbox{\boldmath $\psi$}}}
\def\bfomega{{\mbox{\boldmath $\omega$}}}
\def\bfvarepsilon{{\mbox{\boldmath $\varepsilon$}}}
\def\bfvartheta{{\mbox{\boldmath $\vartheta$}}}
\def\bfvarpi{{\mbox{\boldmath $\varpi$}}}
\def\bfvarrho{{\mbox{\boldmath $\varrho$}}}
\def\bfvarsigma{{\mbox{\boldmath $\varsigma$}}}
\def\bfvarphi{{\mbox{\boldmath $\varphi$}}}
\def\bfimath{{\mbox{\boldmath $\imath$}}}
\def\bfjmath{{\mbox{\boldmath $\jmath$}}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\renewcommand{\L}{\mathbb{L}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\O}{\mathbb{O}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\matlab}{{\sc Matlab} }
\newcommand{\cvec}[1]{{\mathbf #1}}
\newcommand{\rvec}[1]{\vec{\mathbf #1}}
\newcommand{\ihat}{\hat{\textbf{\i}}}
\newcommand{\jhat}{\hat{\textbf{\j}}}
\newcommand{\khat}{\hat{\textbf{k}}}
\newcommand{\minor}{{\rm minor}}
\newcommand{\trace}{{\rm trace}}
\newcommand{\spn}{{\rm Span}}
\newcommand{\rem}{{\rm rem}}
\newcommand{\range}{{\rm range}}
\newcommand{\mdiv}{{\rm div}}
\newcommand{\proj}{{\rm proj}}

\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\attn}[1]{\textbf{#1}}

%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{observation}{Observation}
\newtheorem{note}{Note}
\newtheorem{exercise}{Exercise}
\newcommand{\bproof}{\bigskip {\bf Proof. }}
\newcommand{\eproof}{\hfill\qedsymbol}
\newcommand{\Disp}{\displaystyle}
\newcommand{\qe}{\hfill\(\bigtriangledown\)}
%\setlength{\columnseprule}{1 pt}
\DeclareMathOperator*{\argmin}{arg\,min~}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\st}{subject\,to\,}


\newcommand\red[1]{{\textcolor{red}{#1}}}
\newcommand\blue[1]{{\textcolor{blue}{#1}}}

\newcommand{\todotiny}[1]{\todo[size=\tiny]{#1}}
\newcommand{\todosmall}[1]{\todo[size=\scriptsize]{#1}}

